Two-View Geometry Scoring Without Correspondences

Camera pose estimation for two-view geometry traditionally relies on RANSAC. Normally, a multitude of image correspondences leads to a pool of proposed hypotheses, which are then scored to find a winning model. The inlier count is generally regarded as a reliable indicator of "consensus". We examine this scoring heuristic, and find that it favors disappointing models under certain circumstances. As a remedy, we propose the Fundamental Scoring Network (FSNet), which infers a score for a pair of overlapping images and any proposed fundamental matrix. It does not rely on sparse correspondences, but rather embodies a two-view geometry model through an epipolar attention mechanism that predicts the pose error of the two images. FSNet can be incorporated into traditional RANSAC loops. We evaluate FSNet on fundamental and essential matrix estimation on indoor and outdoor datasets, and establish that FSNet can successfully identify good poses for pairs of images with few or unreliable correspondences. Besides, we show that naively combining FSNet with MAGSAC++ scoring approach achieves state of the art results.

==> tables/E_estimation_scannet.tex <==
% \begin{table}[ht]
% \footnotesize
% \begin{center}
% \begin{tabular}{c c c l c c}
% % \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{MAA at 10\textdegree}} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{Median (\textdegree)}}\\ 
% % \cline{2-3}
% % \cline{5-6}
% % \noalign{\smallskip}
% %  & R & t && $e_R$ & $e_t$\\
% \multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{\maa (R / t)}}\\ 
% \cline{2-6}
% \noalign{\smallskip}
% \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{0-100}} & \multicolumn{1}{c}{} & \multicolumn{2}{c}{\textbf{100-Inf}}\\ 
% \hline \noalign{\smallskip}
% RANSAC w/ SIFT & x.x & x.x && x.x & x.x \\
% MAGSAC++ w/ SIFT & x.x & x.x && x.x & x.x \\
% \ours (F) w/ SIFT & x.x & x.x && x.x & x.x \\
% \hdashline\noalign{\smallskip}
% RANSAC w/ SuperGlue & x.x & x.x && x.x & x.x \\
% MAGSAC++ w/ SuperGlue & 0.29 & 0.19 && \textbf{0.65} & \textbf{0.41} \\
% \ours (F) w/ SuperGlue & 0.28 & 0.18 && 0.63 & 0.38 \\
% \ours (E) w/ SuperGlue & \textbf{0.36} & \textbf{0.23} && 0.60 & 0.33 \\
% \end{tabular}
% \end{center}
% \normalsize
% \caption{\textbf{Essential matrix estimation on ScanNet dataset}. We show that even though \ours is designed for fundamental matrix scoring, we can also used it for evaluating the quality of an Essential matrix hypothesis. We see that \ours trained with Essential matrices (\ours (E)) performs the best in the low number of correspondences split. Interestingly, although the input to the network is the same when evaluating essential or fundamental matrices, specializing \ours to rank one of them is more effective.}
% \label{tab:E_estimation_table}
% \end{table}


\begin{table}[t]
\footnotesize
\begin{center}
\begin{tabular}{c c l c l c}
\multicolumn{1}{c}{} & \multicolumn{3}{c}{\textbf{\maa}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{\mediandeg}}\\ 
\cline{2-4} \cline{6-6}
\noalign{\smallskip}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{0-100}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{All}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{All}}\\
\cline{2-2} \cline{4-4} \cline{6-6}
\noalign{\smallskip}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{R / t } & \multicolumn{1}{c}{} & \multicolumn{1}{c}{R / t}  & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$e_R$ / $e_t$}\\ 
%  & \maa & \mediandeg && \maa & \mediandeg\\
\hline \noalign{\smallskip}
EssNet \cite{zhou2020learn}  & - && ? && ? \\
Map-free \cite{arnold2022map}  & - && 0.39 / 0.13 && 5.75 / 14.20 \\
\hdashline\noalign{\smallskip}
RANSAC \cite{fischler1981random} & 0.27 / 0.16 && 0.37 / 0.24 && 6.55 / 11.68 \\
MAGSAC++ \cite{barath2020magsac++} & 0.29 / 0.19 && 0.40 / 0.26 && 5.95 / 10.96 \\
\ours (F) & 0.28 / 0.18 && 0.38 / 0.24 && 6.34 / 11.70 \\
\ours (E) & \textbf{0.36} / \textbf{0.25} && \textbf{0.44} / \textbf{0.28} && \textbf{5.13} / \textbf{8.96} \\
\ours (F + E) & 0.35 / 0.24 && 0.43 / 0.27 && 5.26 / 9.21 \\
\end{tabular}
\end{center}
\normalsize
\caption{\textbf{Essential matrix estimation on ScanNet dataset}. We see that \ours trained with Essential matrices (\ours (E)) performs the best. Interestingly, although the input to the network is the same when evaluating essential or fundamental matrices, specializing \ours to rank one of them is more effective.}
\label{tab:E_estimation_table}
\end{table}

==> tables/number_its.tex <==

\begin{table}[t]
\footnotesize
\begin{center}
\begin{tabular}{c c l c}
\multicolumn{1}{c}{\textbf{\# Iterations}} & \multicolumn{1}{c}{\textbf{MAA at 10°} (R / t) $\uparrow$} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Median (°)} ($e_R$ / $e_t$) $\downarrow$}\\ 
\hline \noalign{\smallskip}
500 & \textbf{0.38} / \textbf{0.17} && \textbf{6.35} / 17.89 \\
2000 & \textbf{0.38} / \textbf{0.17} && 6.37 / \textbf{17.40} \\
\end{tabular}
\end{center}
\vspace{-1.6em}
\normalsize
\caption{\textbf{MAGSAC++ Fundamental matrix estimation} results on ScanNet test set for different numbers of maximum iterations.}
\label{tab:max_number_its}
\vspace{-1.0em}
\end{table}

==> tables/th_ablation.tex <==

\begin{table}[t]
\footnotesize
\begin{center}
\begin{tabular}{ccccc}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{th=80}} & \multicolumn{1}{c}{\textbf{th=100}} & \multicolumn{1}{c}{\textbf{th=120}} & \multicolumn{1}{c}{\textbf{th=140}}\\ 
\hline \noalign{\smallskip}
MAA (R / t) & \textbf{0.40} / \textbf{0.22} & 0.39 / \textbf{0.22} & 0.39 / \textbf{0.22} & 0.38 / \textbf{0.22}\\
FSNet cases & 58.54\% & 70.44\% & 79.08\% & 84.72\% \\
\end{tabular}
\end{center}
\vspace{-1.6em}
\normalsize
\caption{\textbf{Alternative SP+SG correspondence thresholds for FSNet+MAGSAC++} on ScanNet test set. Note the \% of cases where FSNet is applied. In contrast to the combined method's scores in this table, the MAA score for 100\% FSNet alone are 0.36 / 0.21, and for MAGSAC++ alone are 0.38 / 0.17. }
\label{tab:ablation_th}
% \vspace{-0.8em}
\end{table}

